Towards Measuring Membership Privacy

Machine learning models are increasingly made available to the masses through public query interfaces. Recent academic work has demonstrated that malicious users who can query such models are able to infer sensitive information about records within the training data. Differential privacy can thwart such attacks, but not all models can be readily trained to achieve this guarantee or to achieve it with acceptable utility loss. As a result, if a model is trained without differential privacy guarantee, little is known or can be said about the privacy risk of releasing it. In this work, we investigate and analyze membership attacks to understand why and how they succeed. Based on this understanding, we propose Differential Training Privacy (DTP), an empirical metric to estimate the privacy risk of publishing a classier when methods such as differential privacy cannot be applied. DTP is a measure of a classier with respect to its training dataset, and we show that calculating DTP is efficient in many practical cases. We empirically validate DTP using state-of-the-art machine learning models such as neural networks trained on real-world datasets. Our results show that DTP is highly predictive of the success of membership attacks and therefore reducing DTP also reduces the privacy risk. We advocate for DTP to be used as part of the decision-making process when considering publishing a classifier. To this end, we also suggest adopting the DTP-1 hypothesis: if a classifier has a DTP value above 1, it should not be published.

==> analytical_bound.tex <==
%!TEX root = main.tex
\section{Theoretical Analysis of DTP}

\subsection{Bounds on Optimal Membership Attack}

%TODO:
% 1. What is optimal membership attack
% 2. Exponential binning 
% 3. Theory on bound and proofs

%\begin{Theorem}
%TODO 
% For one target
% prerequisite \epsilon DTP and Pr[logp > log pi + \epsilon] >= exp(epsilon0)
% Conclusion Pr[in]/Pr[out] \leq exp(epsilon0)
%\end{Theorem}

% 3. (optional) experiments to show the bound on Adult dataset 

\subsection{Connection with Differential Privacy}

%TODO DTP maps the possbility by potential "uncertainty sets", differential privacy maps the possibility by noise

% Let $t$ be the target record and $T$ be the target training dataset of size $n$. The data publisher can bound the risk membership inference for $t$ with the following steps. We assume that when the target is in the training set, the probability for class $i$ is

% \begin{equation*}
% p_i = \underset{\substack{T \subseteq D, \\ \mbox{s.t. } t \in T, \left|T\right| = n}}{\mathbb{E}} \left[ p_{\A(T)}(y_i \mid \mathbf{x}_t) \right],
% \end{equation*} 

% and when the target is not in the training set, the probability for class $i$ is

% \begin{equation*}
% p'_i = \underset{\substack{T \subseteq D, \\ \mbox{s.t. } t \in T, \left|T\right| = n}}{\mathbb{E}} \left[ p_{\A(T \setminus \{t\})}(y_i \mid \mathbf{x}_t) \right].
% \end{equation*} 

% Let $\epsilon_i =  \left| \log \frac{p_i}{p'_i} \right|$, and $\DTP(\A,t) = \underset{1 \leq i \leq k}{\max} \epsilon_i$. 

% \textbf{Step 1:} Sample $m$ datasets of size $n-1$ $T_1', T_2', \dots, T_m'$ from $D \setminus \{t\}$, and take $T_j = T_j' \bigcup \{t\}$ for $1 \leq j \leq m$. 

% \textbf{Step 2:} Train classifiers $\A(T_1), \A(T_2), \dots, \A(T_m)$ and \\ $\A(T'_1), \A(T'_2), \dots, \A(T'_m)$ on the sampled datasets. 

% \textbf{Step 3:} Query the features of the target record $\mathbf{x}_t$ on each classifier, and get $p_{ij} = p_{\A(T_j)}(y_i \mid \mathbf{x}_t)$ and $p'_{ij} = p_{\A(T'_j)}(y_i \mid \mathbf{x}_t)$ for all $1 \leq i \leq k$ and $1 \leq j \leq m$. 

% \textbf{Step 4:} For all $1 \leq i \leq k$, calculate $\overline{p}_i$ as the average probability for class $i$ predicted by the $m$ classifiers trained with the target in the dataset and
% % $\sigma_i$ as the sample variance of probability for class $i$ predicted by the $m$ classifiers trained with the target in the dataset. Similarly, calculate
%  $\overline{p}'_i$ as the sample mean when the target record is removed from the training dataset. 

%  Take $\epsilon_0 = \sqrt{-\frac{m*\log\delta}{2}}$ and $\epsilon_{B_i} = \max \left( \left| \log \frac{p_i + \epsilon_0}{p'_i - \epsilon_0 } \right| , \left| \log \frac{p_i - \epsilon_0}{p'_i + \epsilon_0 } \right| \right)$.

% %By Hoeffding inequality, we have $\Pr\left( \left| \overline{p}_i - p_i \right| \geq \epsilon_0 \right) \leq \delta$ and $\Pr\left( \left| \overline{p}'_i - p'_i \right| \geq \epsilon_0 \right) \leq \delta$.
% %\textbf{Step 5:} 
% By Hoeffding inequality, we have $\Pr\left( \epsilon_i > \epsilon_B \right) \leq 2\delta$ for all $1 \leq i \leq k$. 



% %and the sample variance $\sigma_i$ over $p_{i1}, p_{i2}, \dots, p_{im}$. Similarly, calculate $\overline{p}'$ and $\sigma'_i$ over $\sigma_i$ over $p'_{i1}, p'_{i2}, \dots, p'_{im}$.



% %= \frac{1}{m} \sum_{j=1}{m} p_{ij}$ and sample variance $\sigma_i = \frac{1}{m} \frac{(p_{ij} - \overline{p}_i)^2}{m-1}$ and $\overline{p}'_i$ and $\sigma'_i$ over $T_1', T_2', \dots, T_m'$.




==> dp.tex <==
%!TEX root = main.tex
\section{C}

